AuthGuard: Generalizable Deepfake Detection via Language Guidance

Existing deepfake detection techniques struggle to keep-up with the ever-evolving novel, unseen forgeries methods. This limitation stems from their reliance on statistical artifacts learned during training, which are often tied to specific generation processes that may not be representative of samples from new, unseen deepfake generation methods encountered at test time. We propose that incorporating language guidance can improve deepfake detection generalization by integrating human-like commonsense reasoning -- such as recognizing logical inconsistencies and perceptual anomalies -- alongside statistical cues. To achieve this, we train an expert deepfake vision encoder by combining discriminative classification with image-text contrastive learning, where the text is generated by generalist MLLMs using few-shot prompting. This allows the encoder to extract both language-describable, commonsense deepfake artifacts and statistical forgery artifacts from pixel-level distributions. To further enhance robustness, we integrate data uncertainty learning into vision-language contrastive learning, mitigating noise in image-text supervision. Our expert vision encoder seamlessly interfaces with an LLM, further enabling more generalized and interpretable deepfake detection while also boosting accuracy. The resulting framework, AuthGuard, achieves state-of-the-art deepfake detection accuracy in both in-distribution and out-of-distribution settings, achieving AUC gains of 6.15% on the DFDC dataset and 16.68% on the DF40 dataset. Additionally, AuthGuard significantly enhances deepfake reasoning, improving performance by 24.69% on the DDVQA dataset.

==> tables/llava.tex <==
\begin{comment}
\begin{table*}[t!]
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c}
\toprule
                                                                                             & DD-VQA Deepfake Detection & \multicolumn{4}{c}{DD-VQA Answer Generation}                 \\
\midrule
Method                                                                                            & Accuracy                  & BLEU-4         & CIDEr          & ROUGH\_L       & METEOR \\
\midrule                                                                                    
Off-the-shelf LLaVA                                
& 0.6183                    & 0.1422         & 1.4231         & 0.2314         & 0.2489   \\
Fine-tuned LLaVA + fixed vision encoder      &0.7060	 &0.3880	&1.7320	 &0.5470	&0.3212  \\

Fine-tuned LLaVA + plain image token &0.9011	&0.4954	&3.1881	&0.6896	&0.4015\\
Fine-tuned LLaVA + multi-source image tokens(\textbf{Ours}) & \textbf{0.9160}            & \textbf{0.5010} & \textbf{3.2259} & \textbf{0.6910} & \textbf{0.4010} \\
\bottomrule
\end{tabular}
}
\caption{LLaVA ablation study}
\label{tab:llava}
\end{table*}
\end{comment}
